Compressive Demodulation of Mutually Interfering Signals

Multi-User Detection is fundamental not only to cellular wireless communication but also to Radio-Frequency Identification (RFID) technology that supports supply chain management. The challenge of Multi-user Detection (MUD) is that of demodulating mutually interfering signals, and the two biggest impediments are the asynchronous character of random access and the lack of channel state information. Given that at any time instant the number of active users is typically small, the promise of Compressive Sensing (CS) is the demodulation of sparse superpositions of signature waveforms from very few measurements. This paper begins by unifying two front-end architectures proposed for MUD by showing that both lead to the same discrete signal model. Algorithms are presented for coherent and noncoherent detection that are based on iterative matching pursuit. Noncoherent detection is all that is needed in the application to RFID technology where it is only the identity of the active users that is required. The coherent detector is also able to recover the transmitted symbols. It is shown that compressive demodulation requires $\mathcal{O}(K\log N(\tau+1))$ samples to recover $K$ active users whereas standard MUD requires $N(\tau+1)$ samples to process $N$ total users with a maximal delay $\tau$. Performance guarantees are derived for both coherent and noncoherent detection that are identical in the way they scale with number of active users. The power profile of the active users is shown to be less important than the SNR of the weakest user. Gabor frames and Kerdock codes are proposed as signature waveforms and numerical examples demonstrate the superior performance of Kerdock codes - the same probability of error with less than half the samples.

==> intro.tex <==

\section{Introduction}

Demodulation of mutually interfering signals, or Multi-User Detection (MUD) is central to multiaccess communications \cite{verduMUD1998}. It includes the special case of the ``on-off'' Random Access Channel (RAC) \cite{FletcherRanganGoyal2010} that arises in modeling control channels in wireless networks, where active users transmitting their signature waveforms can be modeled as sending $1$'s, and inactive users can be modeled as sending $0$'s. The MUD problem becomes the recovery of the active users, and it may be expanded to demodulation of transmitted symbols from each active user. The two biggest impediments are the asynchronous character of random access and the lack of Channel State Information (CSI) at the Base Station (BS). The signature waveforms of different users are obtained by modulating a chip waveform by digital sequence of length $L$. The total number of users $N$ is severely constrained if all signature waveforms are orthogonal, giving the relationship $N\leq L$. In this paper we are interested in both coherent detection when CSI is known and noncoherent detection when CSI is unknown, under the conditions that the signature waveforms are nonorthogonal and the delays of each user are unknown. 

A baseline architecture for MUD is correlating the received signal with a bank of matched filters \cite{verduMUD1998}, each with respect to a shift of a signature waveform. The first drawback is the huge number of required filters when the number of total users $N$ is large, which is $N_\tau = N (\tau+1)$ where $\tau$ is the maximum delay. A second drawback is that the noise will be colored and amplified by the cross-correlations of selected signature waveforms. An alternative baseline architecture is sampling the received analog signal directly at the chip rate \cite{ApplebaumBajwaDaurteCalderbank2011}. This approach does not amplify the noise but it does require a high-rate Analog-to-Digital Converter (ADC). 

Given that at any time instant the number of active users $K$ is typically small, the promise of Compressive Sensing (CS) \cite{CandesTao2006,Donoho2006} is the demodulation of sparse superpositions of signature waveforms from very few measurements. Therefore MUD can be formulated as a CS problem, and has been considered in \cite{FletcherRanganGoyal2010, XieEldarGoldsmith2011, ZhuGiannakis2011,JinKimRao2010} for synchronous communications; and in \cite{ApplebaumBajwaDaurteCalderbank2011,ApplebaumBajwaDaurte2010} by Applebaum et. al. for asynchronous communications. 

Our contributions in this paper are three-fold. We first demonstrate two front-end architectures for compressive demodulation which can lead to mathematically equivalent discrete signal models. The first architecture is based on subsampling the received signal uniformly at random, which reduces the required rate of ADC in \cite{ApplebaumBajwaDaurteCalderbank2011}. The second architecture is based on a bank of generalized matched filters, which is the extension to asynchronous communication of the architecture for synchronous MUD proposed by Xie et. al. \cite{XieEldarGoldsmith2011} based on analog compressed sensing \cite{MishaliEldar2010}. Another novelty is that both architectures further reduce the number of acquired samples $M$ to be smaller than the length of the signature waveforms $L$, thus reduces the computational complexity of decoding algorithms.


Second, we present coherent detectors to detect both active users and transmitted (BPSK) symbols when the CSI is known, and noncoherent detectors to detect active users when the CSI is unknown. Both algorithms are based on iterative matching pursuit and have taken into accounts the fact that each active user only arrives at one particular delay due to the assumed flat-fading channel model. Our main theoretical contribution is relating the probability of error for the proposed MUD algorithms to two geometric metrics associated with the set of subsampled signature waveforms. These metrics, the worst case and average coherence, were introduced by Bajwa et. al. in the context of model selection \cite{BajwaCalderbankJafarpour2010}.
 We provide explicit  performance guarantees in terms of these coherence metrics and the distribution of received signal powers. These fundamental limits quantify robustness of the compressive MUD algorithms to the ``near-far problem in multiple access communication. 
 it is shown compressive demodulation requires $\mathcal{O}(K\log N(\tau+1))$ samples to recover $K$ active users whereas standard MUD requires $N(\tau+1)$ samples to process $N$ total users with a maximal delay $\tau$
The average coherence of full Gabor frames is calculated in \cite{BajwaCalderbankJafarpour2010} and here we extend this analysis to the subsampled Gabor frames. 
We demonstrate through simulation that our compressive MUD architecture and algorithms are able to support more users at a given number of measurements (which corresponds to the number of correlators in the mixing of signal architecture or the sampling rate in the chip-rate sampling architecture). We also describe how our methods can be extended to support demodulation of symbols in the absence of Channel State Information, which enables blind MUD.
the Performance guarantees for both algorithms are provided which allow managing $K$ active users from $\mathcal{O}(K\log N_{\tau})$ samples.
 


Finally, we consider codeword designs that satisfies the  signature waveforms:
\cite{VerduShamai1999,ViswanathAnantharam1999,TroppDhillonHeath2004}

 




The rest of the paper is organized as follows.

